Creating multicomponent Schr\"odinger cat states in a coupled qubit-oscillator system

We present a method for preparing various exotic modifications of Schr{\"o}dinger cat states by coupling a semiclassical oscillator to a system of qubits. Varying the number of qubits and parameters of the protocol (involving quantum quench of the coupled system and a subsequent spin measurement), we bring the oscillator into a coherent superposition composed of an arbitrary number of wavepackets in tunable proportions and motion relations. The method can be implemented with the aid of current experimental techniques and may find applications in quantum information and sensing protocols.

==> defs.tex <==
\DeclareMathOperator{\e}{e}
\DeclareMathOperator{\tg}{tg}
\DeclareMathOperator{\cotg}{cotg}
\DeclareMathOperator{\arccotg}{arccotg}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\gradient}{grad}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\real}{Re}
\DeclareMathOperator{\imaginary}{Im}
\DeclareMathOperator{\Ai}{Ai}
\DeclareMathOperator{\Bi}{Bi}
\DeclareMathOperator{\Tp}{\mathsf{T}}

\def\sizeN{\mathcal{N}}

\renewcommand{\d}{\mathrm{d}}
\newcommand{\D}{\mathcal{D}}

\def\O#1{\mathcal{O}\left({#1}\right)}

\def\superket#1{\left|{#1}\right)}
\def\superbra#1{\left({#1}\right|}
\def\superbraket#1#2{\left({#1}\middle|{#2}\right)}

\def\superoperator#1{\hat{\mathcal{#1}}}

\def\ket#1{\left|{#1}\right\rangle}
\def\bra#1{\left\langle{#1}\right|}
\def\mean#1{\left\langle{#1}\right\rangle}
\def\braket#1#2{\left\langle{#1}\middle|{#2}\right\rangle}
\def\matrixelement#1#2#3{\left\langle{#1}\middle|{#2}\middle|{#3}\right\rangle}
\def\ketbra#1#2{\left|{#1}\middle\rangle\middle\langle{#2}\right|}
\def\projector#1{\left|{#1}\middle\rangle\middle\langle{#1}\right|}
\def\uncertainty#1#2{\Delta_{#1}{\operator{#2}}^{2}}
\def\diagonal#1{\,\text{diag}\left(#1\right)}

\def\freg{f_\mathrm{reg}}

\def\c{,\!}
\def\unit#1{\,\mathrm{#1}}

\def\hi#1{^{({#1})}}

\def\clebsch#1#2#3#4#5#6{\mathcal{C}^{#5\,#6}_{#1\,#2\:#3\,#4}}
\def\threej#1#2#3#4#5#6{\begin{pmatrix}#1&#2&#3\\#4&#5&#6\end{pmatrix}}

\def\commutator#1#2{\left[{#1},{#2}\right]}
\def\anticommutator#1#2{\left\{{#1},{#2}\right\}}
\def\associator#1#2#3{\left[{#1},{#2},{#3}\right]}
\def\poisson#1#2{\left\{{#1},{#2}\right\}}

\def\abs#1{\left\lvert{#1}\right\rvert}
\def\abss#1{\left|{#1}\right|^{2}}							% Square of the absolute value
\def\norm#1{\left\lVert{#1}\right\rVert}
\def\intinf{\int_{-\infty}^{\infty}}						% Infinite integral

\def\minus#1{\left(-1\right)^{#1}}
%\def\ui#1{(#1)}
\def\ti#1{\mathrm{#1}}										% Text index

\def\error#1{{\color{red}{\bf{#1}}}}
\def\trick#1{{\color{blue}#1}}

\def\hilbert#1{\mathcal{#1}}								% Hilbert space
\def\group#1{\mathrm{#1}}									% Group
\def\algebra#1{\mathrm{#1}}
\def\ensemble#1{\mathsf{#1}}

\def\vector#1{\boldsymbol{#1}}								% Vector
\def\matrix#1{\mathsf{#1}}										% Matrix
\def\axis#1{\mathrm{#1}}

\def\2F1#1#2#3#4{\,{}_{2}F_{1}\!\left(#1,#2,#3;#4\right)}
\def\1F1#1#2#3{\,{}_{1}F_{1}\!\left(#1,#2;#3\right)}

\def\operator#1{\mathsf{\hat{#1}}}
\def\vectoroperator#1{\boldsymbol{\mathsf{\hat{#1}}}}
\def\tensoroperator#1#2{\hat{\mathbb{#1}}^{(#2)}}					% tensor operator
\def\tensoroperatorcomponent#1#2#3{\hat{\mathsf{#1}}^{(#2)}_{#3}}	% tensor operator - component
\def\reducedmatrixelement#1#2#3{\left(#1\middle\lVert#2\middle\rVert#3\right)}	    % Reduced matrix element

\def\propagator{G(\vx_{\rf},t_{\rf};\vx_{\ri},t_{\ri})}

\newcommand{\partialderivative}[3][]{\ifthenelse{\isempty{#1}}	% Partial derivative
	{\frac{\partial{#2}}{\partial{#3}}}
	{\frac{\partial^{#1}{#2}}{\partial{#3}^{#1}}}
}

\newcommand{\derivative}[3][]{\ifthenelse{\isempty{#1}}	% Normal derivative
	{\frac{\d{#2}}{\d{#3}}}
	{\frac{\d^{#1}{#2}}{\d{#3}^{#1}}}
}

\def\conjugate#1{{#1}^{\dagger}}
\def\transpose#1{{#1}^{\intercal}}

\def\operatorconjugate#1{\conjugate{\operator{#1}}}

\def\makematrix#1{\begin{pmatrix}#1\end{pmatrix}}       % Matrix
\def\Vdots{\vphantom{0}\smash[t]{\vdots}}

\def\equationcomment#1{\begin{vmatrix}#1\end{vmatrix}}  % Comment in equation (e.g. substitution in integral)

\long\def\important#1{\boxed{#1}}

\def\MeV{\mathrm{MeV}}
\def\im{\mathrm{i}}
\def\const{\mathrm{const}}

\def\ie{{\it i.e., }}

\def\filecopy#1#2{
	\IfFileExists{#1}{
		\newwrite\copyfile  % open the file to write to
		\immediate\openout\copyfile=#2

		\newread\file      % open the file to read from
		\openin\file=#1

		\begingroup\endlinechar=-1
		\loop\unless\ifeof\file
		\read\file to\fileline  % Read one line and store it into \fileline
		%  \fileline\par                   % print the content into the pdf
		\immediate\write\copyfile{\unexpanded\expandafter{\fileline}}  % print the content to copy.txt
		\repeat
		\endgroup
	}{}
}

